Inverse Global Illumination using a Neural Radiometric Prior

Inverse rendering methods that account for global illumination are becoming more popular, but current methods require evaluating and automatically differentiating millions of path integrals by tracing multiple light bounces, which remains expensive and prone to noise. Instead, this paper proposes a radiometric prior as a simple alternative to building complete path integrals in a traditional differentiable path tracer, while still correctly accounting for global illumination. Inspired by the Neural Radiosity technique, we use a neural network as a radiance function, and we introduce a prior consisting of the norm of the residual of the rendering equation in the inverse rendering loss. We train our radiance network and optimize scene parameters simultaneously using a loss consisting of both a photometric term between renderings and the multi-view input images, and our radiometric prior (the residual term). This residual term enforces a physical constraint on the optimization that ensures that the radiance field accounts for global illumination. We compare our method to a vanilla differentiable path tracer, and more advanced techniques such as Path Replay Backpropagation. Despite the simplicity of our approach, we can recover scene parameters with comparable and in some cases better quality, at considerably lower computation times.

==> figsrc/train_curves.tex <==
\begin{figure}
\vspace{-2mm}
    \centering
    \includegraphics[width = 0.48\textwidth]{Figures/curves_hour_prbdebugged.pdf}
    \caption{%\fabrice{Give the time in hours instead of seconds in the right column and ``Time (hours)'' instead of ``Timestamp (hours)''.} 
    \textbf{Reconstruction accuracy}. Albedo, roughness and photometric error, for the \Staircase scene,  as a function of training steps and time. 
    %Despite using short paths, 
    Our method correctly accounts for global illumination thanks to our neural radiometric prior, resulting in high accuracy at low computational cost.} 
    
    
    
    %The sampling rate here was reduced to 14 (instead of 16 in other ) to keep peak memory usage within our GPU budget. 
%    \fabrice{Why is the ``PRB'' line shorter in the left column? Why is the ``Direct'' line not longer if it has a lower sampling rate? I thought it would have more training steps in order to have the same number of total samples.}\saeed{Everything has equal sampling rate of 14 sample per pixel, I repeated this experiment with spp=14 across all methods (so that AD fits in memory and we can have plots of the same length). PRB fixed}}
%    \caption{\textbf{Optimization curves.} The curves show the error of albedo (top), roughness (middle) and the photometric loss(bottom) against  training step and time for the \Staircase. The y axis in all plots is \emph{log-scale}. The setting in these experiments is the same as in Figures \ref{fig:teaser} and \ref{fig:main_results} and Table \ref{tab:performance}, with the only exception that during the optimization we use 14 spp for candidate images instead of 16 spp, because at the latter setting AD kept running out of memory.}
    \label{fig:curves}
    \vspace{-3mm}
\end{figure}

==> table/performance_table.tex <==
\newcommand{\perfTimeDirect}{0.4754}
\newcommand{\perfTensorTimeDirect}{0.3145}
\newcommand{\perfMitsubaTimeDirect}{0.3258}
\newcommand{\perfTimeAD}{3.8422}
\newcommand{\perfTensorTimeAD}{2.7752}
\newcommand{\perfMitsubaTimeAD}{2.1767}
\newcommand{\perfTimePRB}{6.5176}
\newcommand{\perfTensorTimePRB}{3.9690}
\newcommand{\perfMitsubaTimePRB}{3.2239}
\newcommand{\perfTimeOursNoSec}{0.5649}
\newcommand{\perfTensorTimeOursNoSec}{0.4003}
\newcommand{\perfMitsubaTimeOursNoSec}{0.3911}
\newcommand{\perfTimeOurs}{0.9661}
\newcommand{\perfTensorTimeOurs}{0.7610}
\newcommand{\perfMitsubaTimeOurs}{0.7377}
\newcommand{\perfTensorTimeOursGrid}{0.6364}
\newcommand{\perfMitsubaTimeOursGrid}{0.6078}
\newcommand{\perfTensorTimeOursNoSecGrid}{0.3372}
\newcommand{\perfMitsubaTimeOursNoSecGrid}{0.3383}

\newcommand{\perfVRamDirect}{11779}
\newcommand{\perfRamDirect}{836}
\newcommand{\perfTensorVRamDirect}{5463}
\newcommand{\perfTensorRamDirect}{288}
\newcommand{\perfMitsubaVRamDirect}{6729}
\newcommand{\perfMitsubaRamDirect}{316}
\newcommand{\perfVRamAD}{23911}
\newcommand{\perfRamAD}{1184}
\newcommand{\perfTensorVRamAD}{7037}
\newcommand{\perfTensorRamAD}{955}
\newcommand{\perfMitsubaVRamAD}{7867}
\newcommand{\perfMitsubaRamAD}{902}
\newcommand{\perfVRamPRB}{10003}
\newcommand{\perfRamPRB}{2698}
\newcommand{\perfTensorVRamPRB}{5439}
\newcommand{\perfTensorRamPRB}{652}
\newcommand{\perfMitsubaVRamPRB}{6723}
\newcommand{\perfMitsubaRamPRB}{1240}
\newcommand{\perfVRamOursNoSec}{11815}
\newcommand{\perfRamOursNoSec}{852}
\newcommand{\perfTensorVRamOursNoSec}{7435}
\newcommand{\perfTensorRamOursNoSec}{858}
\newcommand{\perfMitsubaVRamOursNoSec}{8759}
\newcommand{\perfMitsubaRamOursNoSec}{893}
\newcommand{\perfVRamOurs}{17903}
\newcommand{\perfRamOurs}{1020}
\newcommand{\perfTensorVRamOurs}{8887}
\newcommand{\perfTensorRamOurs}{1016}
\newcommand{\perfMitsubaVRamOurs}{9667}
\newcommand{\perfMitsubaRamOurs}{1044}
\newcommand{\perfVRamOursGrid}{17903}
\newcommand{\perfRamOursGrid}{1020}
\newcommand{\perfTensorVRamOursGrid}{6475}
\newcommand{\perfTensorRamOursGrid}{467}
\newcommand{\perfMitsubaVRamOursGrid}{8645}
\newcommand{\perfMitsubaRamOursGrid}{536}
\newcommand{\perfVRamOursNoSecGrid}{11815}
\newcommand{\perfRamOursNoSecGrid}{852}
\newcommand{\perfTensorVRamOursNoSecGrid}{6265}
\newcommand{\perfTensorRamOursNoSecGrid}{313}
\newcommand{\perfMitsubaVRamOursNoSecGrid}{8537}
\newcommand{\perfMitsubaRamOursNoSecGrid}{369}


\begin{table}
\centering
\small
\caption{
\textbf{Performance comparison.} We compare the per-step time in seconds and peak GPU memory in MB (VRAM) for the \Staircase scene. \textbf{Main results:} the MLP columns use an MLP to model SVBRDF parameters. %We use an MLP to represent the radiance field in \textbf{Ours-1B} and \textbf{Ours}, where we compute a one bounce and extra bounce prior, respectively. By the same token, \textbf{Ours-Grid-1B} and \textbf{Ours-Grid} differ in the number of prior bounces, but they use a 3D texture representation for radiance.
Our method runs significantly faster than AD and PRB thanks to tracing shorter paths. The '1B' after our method represents a one bounce prior. \textbf{Overhead analysis:} The columns/rows under `Mitsuba Grid' use a Mitsuba dense grid for the scene parameters, hence these techniques are implemented entirely within Mitsuba. They reveal the amount of overhead incurred by cross-library computation when using an MLP for the scene parameters.
}
\begin{tabular}{lccccc}
    \toprule
    {} & \multicolumn{2}{c}{MLP} && \multicolumn{2}{c}{Mitsuba Grid} \\
        \cmidrule{2-3}\cmidrule{5-6}
    {} & Time & Peak VRAM && Time & Peak VRAM \\
    \midrule
    
%\begin{tabular}{lccccc}
    %\toprule
    %{} & \multicolumn{2}{c}{MLP} && \multicolumn{2}{c}{Mitsuba Grid} \\
    %\cmidrule{2-3}\cmidrule{5-6}
    %{} & Time & Peak VRAM && Time & Peak VRAM \\
    %\midrule

AD-Direct & \perfTimeDirect & \perfVRamDirect &  & \perfMitsubaTimeDirect & \perfMitsubaVRamDirect \\
AD-PT & \perfTimeAD & \perfVRamAD &  & \perfMitsubaTimeAD & \perfMitsubaVRamAD \\
PRB & \perfTimePRB & \perfVRamPRB &  & \perfMitsubaTimePRB & \perfMitsubaVRamPRB \\

\midrule

AD-Ours-1B & \perfTimeOursNoSec & \perfVRamOursNoSec &  & \perfMitsubaTimeOursNoSec & \perfMitsubaVRamOursNoSec \\
AD-Ours & \perfTimeOurs & \perfVRamOurs &  & \perfMitsubaTimeOurs & \perfMitsubaVRamOurs \\

\midrule

AD-Ours-Grid-1B & - & - &  & \perfMitsubaTimeOursNoSecGrid & \perfMitsubaVRamOursNoSecGrid \\
AD-Ours-Grid & - & - &  & \perfMitsubaTimeOursGrid & \perfMitsubaVRamOursGrid \\
\bottomrule

\end{tabular}
\label{tab:performance}
\end{table}

==> x-scratch.tex <==


\matthias{remove entire section; add any necessary explanations to section about our method}

\jan{Use eqref instead of ref for referencing equations. \saeed{resolved}}
\jan{I don't like capitalizing the names of methods in text, because it is hard to draw the line between when to still capitalize and when not (e.g. what do you do for the rendering equation). Using low-caps is hassle free.}
Neural Radiosity \cite{hadadan2021neural} proposes to find a solution of the rendering equation (Equation \eqref{eq:rendering-equation}) using a neural network. The radiance function $L(x,\omega_o)$ in Equation \eqref{eq:rendering-equation} is represented by a neural network with a set of parameters $\theta$, denoted as $L_{\theta}(x,\omega_o)$, that takes location $x$ and direction $\omega_o$ and spits out the outgoing radiance. The parameters $\theta$ of this network can be directly optimized by minimizing the norm  of the \emph{residual} of the rendering equation.
\jan{This needs to be introduced more gently. We shouldn't expect readers to know Neural Radiosity.}\saeed{Added more details}
The residual $r_{\theta}(x,\omega_o)$ is
%
\begin{dmath}
\label{eq:renderingresidual}
    r_{\theta}(x,\omega_o) =  L_{\theta}(x,\omega_o) - E(x,\omega_o) \nonumber \\
     - \int_{\mathcal{H}^2} f(x,\omega_i, \omega_o) L_{\theta}(x'(x,\omega_i),-\omega_i) d\omega_i^{\perp},
\end{dmath}
%
which is simply the difference between the left and right-hand sides of Equation \eqref{eq:rendering-equation} when the radiance function $L$ is substituted by $L_{\theta}$. Monte Carlo sampling is used to repeatedly estimate the norm of the residual as in
%
\begin{align}
    \mathcal{L}(\theta) \approx \frac{1}{N}\sum_{j=1}^{N} \frac{r_{\theta}(x_j,\omega_{o,j})^2}{p(x_j,\omega_{o,j})},
\end{align}
%
where $N$ is the number of samples, and samples of surface locations $x_j$ and outgoing directions $\omega_{o,j}$ are distributed according to probability density $p(x,\omega)$.

%the MC approximation of the gradient $\nabla_{\theta} \mathcal{L}(\theta)$ is
%
%\begin{align}
%\label{eq:residualsampling}
%\nabla_{\theta} \mathcal{L}(\theta) \approx& \frac{1}{N}\sum_{j=1}^{N} \frac{2 r_{\theta}(x_j,\omega_{o,j}) \nabla_{\theta} r_{\theta}(x_j,\omega_{o,j})}{p(x_j,\omega_{o,j})},
%\end{align}
% %

Assuming that the BRDF term is not dependent on $\theta$, 
the gradient of the residual is
% %
\begin{align}
\nabla r_{\theta}(x,\omega_o) = &  \nabla L_{\theta}(x,\omega_o) - \nonumber \\
&\int_{\mathcal{H}^2} f(x,\omega_i, \omega_o)  L_{\theta}(x'(x,\omega_i),-\omega_i) d\omega_i^{\perp}.
\end{align}
%

Neural Radiosity is a self-training approach, that is, there is no use of ground truth data to supervise the training. \jan{We need to mention this is the radiometric prior that we are leveraging to link it back to the intro.}\saeed{resolved}
A pre-trained instance of this network can serve as a compact, re-renderable, and view-independent solution of the rendering equation. Additionally, such a solution would be accounting for global illumination effects, which is why the residual term is the radiometric prior we use in this paper.

During the inference, one could directly query the radiance network at the primary surface intersection of camera rays,
%
\begin{dmath}
\label{eq:LHS-measurement-equation}
I_k^{LHS} = \int_{\mathcal{A}}\int_{\mathcal{H}^2} W_k(x,\omega) L_\theta(x,\omega) dx d\omega^{\perp},
\end{dmath}
which they call a left hand side (LHS) rendering. Alternatively, one could substitute the term $L_{\theta}$ with the right side of the rendering equation, and get
%
\begin{dmath}
\label{eq:RHS-measurement-equation}
I_k^{RHS} = \int_{\mathcal{A}}\int_{\mathcal{H}^2} W_k(x,\omega) . ( E(x,\omega_o) + \\
\int_{\mathcal{H}^2} f(x,\omega_i, \omega_o) L_{\theta}(x'(x,\omega_i),-\omega_i) d\omega_i^{\perp} dx) d\omega^{\perp},
\end{dmath}
which is called a RHS rendering. Ideally, in the presence of a perfectly optimized network with $r_{\theta}(x,\omega_o) = 0$ everywhere, these renderings should be identical; in practice, where a residual equal to zero is hard to achieve, a RHS rendering would be more accurate than LHS, because it queries the network one bounce further from the camera, i.e. there is an additional MC estimator of the inner-most integral $L_{\theta}$, which reduces the impact of the approximation errors of $L_{\theta}$ at the cost of increased variance.
\jan{Could mention that on the RHS, the network is queried one bounce further from the camera, i.e. there is an additional MC estimator of the inner-most integral $L_{\theta}$, which reduces the impact of the approximation errors of $L_{\theta}$ at the cost of increased variance}\saeed{Replaced the text.}







Our method is based on Neural Radiosity for primal rendering, 
%and uses automatic differentiation for backward propagation of the gradients to the scene parameters. Similar to Neural Radiosity,
where we parameterize a radiance network using a parameter set $\theta$, $L_{\theta}$ using which we compute RHS renderings as candidate images (Equation \ref{eq:RHS-measurement-equation}). The candidate image is then compared to a ground truth in a Reconstruction loss, and the gradient of the loss is backpropagated to the scene parameters using a vanilla AD backward mode. Thus, we define the reconstruction loss as
%
\begin{align}
    \mathcal{L}_{recons}(\phi)= \left\|I^{RHS} - gt\right\|^2
    \label{eq:recons-loss}
\end{align}
%
where $\phi$ is the set of scene parameters being optimized. In order to train the radiance network, we borrow the loss function from the original paper, i.e. the norm of the residual (Equation \ref{eq:renderingresidual}) as the loss function,
%
\begin{align}
\mathcal{L}_{residual}(\theta) &= \left\| r_{\theta}(x,\omega_o) \right\|_2^2 \nonumber \\
&= \int_{\mathcal{M}}\int_{\mathcal{H}^2} r_{\theta}(x,\omega_o)^2 dxd\omega_o. 
\label{eq:residual-loss}
\end{align}
%
This loss term is the \emph{radiometric prior} that serves as a physical condition by which we condition the inverse rendering to account for global illumination in the scene.

Finally, we minimize the sum of the two losses as the training loss,
\begin{align}
\mathcal{L}(\phi, \theta) &= \mathcal{L}_{recons}(\phi) + \mathcal{L}_{residual}(\theta).
\label{eq:complete-loss}
\end{align}

